PICBench: Benchmarking LLMs for Photonic Integrated Circuits Design

While large language models (LLMs) have shown remarkable potential in automating various tasks in digital chip design, the field of Photonic Integrated Circuits (PICs)-a promising solution to advanced chip designs-remains relatively unexplored in this context. The design of PICs is time-consuming and prone to errors due to the extensive and repetitive nature of code involved in photonic chip design. In this paper, we introduce PICBench, the first benchmarking and evaluation framework specifically designed to automate PIC design generation using LLMs, where the generated output takes the form of a netlist. Our benchmark consists of dozens of meticulously crafted PIC design problems, spanning from fundamental device designs to more complex circuit-level designs. It automatically evaluates both the syntax and functionality of generated PIC designs by comparing simulation outputs with expert-written solutions, leveraging an open-source simulator. We evaluate a range of existing LLMs, while also conducting comparative tests on various prompt engineering techniques to enhance LLM performance in automated PIC design. The results reveal the challenges and potential of LLMs in the PIC design domain, offering insights into the key areas that require further research and development to optimize automation in this field. Our benchmark and evaluation code is available at https://github.com/PICDA/PICBench.

==> Makefile <==
ENGINE := pdflatex
BIB := bibtex

PROJECT := DATE25-PIC-Routing

all:
	@$(ENGINE) $(PROJECT).tex
	@$(BIB)    $(PROJECT)
	@$(BIB)    $(PROJECT)
	@$(ENGINE) $(PROJECT).tex
	@$(ENGINE) $(PROJECT).tex

fast:
	@$(ENGINE) $(PROJECT).tex

bib:
	@$(BIB)    $(PROJECT)

clean:
	@$(RM) -rf *.log *.aux *.blg *.bbl *.gz *.dvi *.thm *.dat *.out *latexmk *fls *busy\)


==> acm-setting.tex <==
\usepackage{amsmath,amsfonts}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{amsthm}
\usepackage{listings}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{cleveref}
\usepackage{booktabs}
\usepackage{comment}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{bm}
\usepackage{url}
\usepackage{xspace}
\usepackage{pifont}
\usepackage{arydshln}
\usepackage{verbatim}
\usepackage[referable]{threeparttablex}
\usepackage{calc} 
%\usepackage{ulem}
\usepackage{color}
\usepackage{float}
\usepackage{stfloats}
\usepackage{subcaption}
% \usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage[utf8]{inputenc}
\usepackage{booktabs} % For prettier tables
\usepackage{tabularx} % For tables with adjustable-width columns
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage[utf8]{inputenc}
% \usepackage[english]{babel}
%\usepackage{etoolbox}
%\appto\TPTnoteSettings{\footnotesize} % make table notes smaller
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}
\thispagestyle{empty}

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]

\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{scalefnt}
\pgfplotsset{compat=newest}
\newcommand{\true}{\top}
\newcommand{\false}{\bot}
\newcommand{\Tr}{\mathit{Tr}}
\newcommand{\Prop}{\mathit{P}}
\newcommand{\tp}{\mathit{t_p}}
\newcommand{\tl}{\mathit{t_l}}
\newcommand{\Var}{{\mathit{Var}}}
\newcommand{\V}{{\mathit{Var}}}
\newcommand{\Vp}{{\mathit{Var'}}}
\newcommand{\Cnstr}{{\mathit{C}}}
\newcommand{\D}{{\mathit{D}}}
\newcommand{\I}{{\mathit{I}}}
%\newcommand{\U}{{\mathit{U}}}
\newcommand{\Up}{{\mathit{U'}}}
\newcommand{\rfmap}{{\mathit{r}}}
\newcommand{\Init}{\mathit{Init}}
\newcommand{\Trans}{\mathit{Tr}}
\newcommand{\Bad}{\mathit{Bad}}
\newcommand{\Expr}{\mathit{Expr}}
\newcommand{\Inv}{\mathit{Inv}}
\newcommand{\base}{\mathit{base}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\THeshold}{\mathit{Th}}
\newcommand{\tensor}[1]{\mathcal{#1}}      % define tensor command
\renewcommand{\vec}[1]{\boldsymbol{#1}}    % re-define vec command

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{USTgold}{RGB}{153,102,0}
\definecolor{USTyellow}{RGB}{204,153,0}
\definecolor{USTyellowlight}{RGB}{255,212,0}
\definecolor{USTorange}{RGB}{255,166,26}
\definecolor{USTpink}{RGB}{255,157,157}
\definecolor{USTblue}{RGB}{0,51,102}
\definecolor{USTmiddle}{RGB}{0,116,188}
\definecolor{USTlight}{RGB}{99,202,225}
\definecolor{USTgray}{RGB}{204,204,204}
\definecolor{USTred}{RGB}{237,27,47}
\definecolor{USTdarkred}{RGB}{124,35,72}

\definecolor{CUHKorange}{RGB}{244,106,18} %F47012
\definecolor{CUHKblue}{RGB}{0,111,190}    %006FBE
\definecolor{CUHKgreen}{RGB}{0,127,128}   %007F80
\definecolor{CUHKred}{RGB}{228,46,36}     %E42E24
\definecolor{CUHKyellow}{RGB}{198,148,34} %C69422
\definecolor{CUHKdark}{RGB}{114,44,114}   %722C72
\definecolor{CUHKmiddle}{RGB}{144,44,144} %902C90
\definecolor{CUHKlight}{RGB}{167,44,167} 


\newcommand{\deftitle}[0]{{\texttt{E-Syn}}\xspace}
\newcommand{\deftextEsyn}[0]{\mbox{\texttt{E-Syn}}\xspace}

\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}{Corollary}%[theorem]
\newtheorem{lemma}[theorem]{Lemma}

\iftrue
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\setlength{\columnsep}{14pt}                               % set space between columns
\fi

\acmConference[DAC '24]{Design Automation Conference}{June 23--27, 2024}{San Francisco, CA}

\newcommand{\minisection}[1]{\vspace{.06in}\noindent{\textbf{#1}}}

% ==== page margin settings
\iftrue
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=50pt, bottom=72pt, inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\fi

\iftrue
% === shrink page num
\usepackage{titlesec}
\titlespacing\section{2pt}{5pt plus 1pt minus 1pt}{0pt plus 1pt minus 1pt}
\titlespacing\subsection{2pt}{5pt plus 1pt minus 1pt}{0pt plus 1pt minus 1pt}
\titlespacing\subsubsection{2pt}{5pt plus 1pt minus 1pt}{2pt plus 1pt minus 1pt}
\usepackage[inline]{enumitem}
\setlist{leftmargin=5.08mm}
\fi

\iftrue
\setlength{\textfloatsep}{3pt plus 1pt minus 1pt}          % set space between float and text
\setlength{\floatsep}{3pt plus 1pt minus 1pt}              % set space between two floats
\setlength{\intextsep}{3pt plus 1pt minus 1pt}             % set space between text and float
\setlength{\columnsep}{16pt}                               % set space between columns
% ==== reduce space around equations
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{2pt} \setlength{\abovedisplayshortskip}{2pt}
\fi


